DPMC: Weighted Model Counting by Dynamic Programming on Project-Join Trees

We propose a unifying dynamic-programming framework to compute exact literal-weighted model counts of formulas in conjunctive normal form. At the center of our framework are project-join trees, which specify efficient project-join orders to apply additive projections (variable eliminations) and joins (clause multiplications). In this framework, model counting is performed in two phases. First, the planning phase constructs a project-join tree from a formula. Second, the execution phase computes the model count of the formula, employing dynamic programming as guided by the project-join tree. We empirically evaluate various methods for the planning phase and compare constraint-satisfaction heuristics with tree-decomposition tools. We also investigate the performance of different data structures for the execution phase and compare algebraic decision diagrams with tensors. We show that our dynamic-programming model-counting framework DPMC is competitive with the state-of-the-art exact weighted model counters cachet, c2d, d4, and miniC2D.

==> old/3-jointrees.tex <==
\section{Join trees of CNF formulas}

Given a CNF formula, we can construct a join tree, which specifies an order to apply projection and multiplication operations for model counting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Join Trees and Factor Graphs}

A join tree is a generalization of variable elimination on a factor graph as presented in the algorithm below.

\begin{algorithm*}[H]
\caption{Variable elimination on a factor graph}
    \DontPrintSemicolon
    \KwIn{$X$: set of $m \ge 1$ Boolean variables}
    \KwIn{$g : 2^X \to \B$: function with factorization $g = \prod_{i = 1}^l f_i$ where $f_i : 2^{A_i} \to \B$ with $\bigcup_{i = 1}^l A_i = X$}
    \KwOut{$\proj_X g : 2^\emptyset \to \N$: marginalization of $g$}
    $F \gets \set{f_1, f_2, \ldots, f_l}$\;
    $x_1, x_2, \ldots, x_m \gets$ variables ordered optimally or heuristically\;
    \For{$j = 1, 2, \ldots, m$}{
        $S \gets \set{f_i \in F : x_j \in A_i}$\;
        $f_k \gets \proj_{x_j} \prod_{f_i \in S} f_i$
            \tcc*{new factor $f_k$ with $A_k = \bigcup_{f_i \in S} A_i \setminus \set{x_j}$}
        $F \gets F \cup \set{f_k}$\;
        $F \gets F \setminus S$\;
    }
    $f \gets$ the only factor remaining in $F$\;
    \Return{$f$}
\end{algorithm*}

Variable elimination sums out exactly one variable $x_j$ in each iteration.
A join tree is more general as it allows for the projection of several variables (in a set $P_i$) at once.


==> old/A-DPDB.tex <==
\section{Weighted Model Counting with Nice Tree Decompositions}

See the algorithm below, a weighted version of the dynamic-programming model-counting algorithm in \cite{fichte2020exploiting}.

\begin{algorithm}%[H]
\caption{Literal-weighted CNF model counting with nice TD}
    \DontPrintSemicolon
    \KwData{$X$: set of Boolean variables}
    \KwData{$W^0, W^1 : X \to \R$: weight functions for negative and positive literals}
    \KwData{$\phi : 2^X \to \B$: CNF formula}
    \KwData{$\Delta = (T, \chi)$: nice TD of $\phi$}
    \KwIn{$t$: node in rooted binary tree $T$}
    \KwIn{$\chi(t) \subseteq X$: bag}
    \KwIn{$\phi_t = \set{\kappa \in \phi : \vars(\kappa) \subseteq \chi(t)}$}
    \KwOut{$\tau_t = \set{\seq{I, c} : I \in 2^{\vars(\phi_t)} \wedge c \in \R}$: table of assignments and corresponding weighted model counts}
    % \Begin{
            \If{$t$ is \emph{leaf}}{
                $\tau_t \gets \set{\seq{\emptyset, 1}}$ \\
                    % \tcc*{builds ADD $A$ for cluster $\kappa_i$}
            }
            \ElseIf{$t$ is \emph{intro} and $\C(t) = \set{t'}$ and $\chi(t) \setminus \chi(t') = \set{a}$}{
                $\tau_t \gets \set{
                    \seq{I \cup \set{a \mapsto 0}, c \mult \phi_t(I[a \mapsto 0]) \mult W^0(a)},
                    \seq{I \cup \set{a \mapsto 1}, c \mult \phi_t(I[a \mapsto 1]) c \mult W^1(a) } :
                    \seq{I, c} \in \tau_{t'}
                }$
            }
            \ElseIf{$t$ is \emph{removal} and $\C(t) = \set{t'}$ and $\chi(t') \setminus \chi(t) = \set{a}$}{
                $\tau_t \gets \set{\seq{I, c_0 + c_1} : \seq{I \cup \set{a \mapsto 0}, c_0}, \seq{I \cup \set{a \mapsto 1}, c_1} \in \tau_{t'}}$
            }
            \ElseIf{$t$ is \emph{join} and $\C(t) = \set{t', t''}$}{
                $\tau_t \gets \set{\seq{I, c' \mult c''} : \seq{I, c'} \in \tau_{t'} \wedge \seq{I, c''} \in \tau_{t''}}$
            }
            \Else{Error: $\Delta$ is not nice}
            \Return{$A(\emptyset)$}
    % }
\end{algorithm}


==> old/A-examples.tex <==





\section{Examples}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{CNF Formula}

In propositional logic, a literal is a Boolean variable or its negation.
A clause is a disjunction of
% one or more
literals.
A CNF formula is a conjunction of
% one or more
clauses.
Equation \eqref{eq_cnf} illustrates a CNF formula $\phi$.
\begin{align}
    \phi = \pars{x_1 \vee x_3} \wedge \pars{\neg x_1 \vee \neg x_3} \wedge x_2 \wedge \pars{x_3 \vee x_4} \wedge \neg x_4 \wedge x_5
    \label{eq_cnf}
\end{align}

See Listing \ref{formatCNF} for the CNF file format.

\begin{lstlisting}[float=*, firstline=2, caption={The CNF formula in Equation \eqref{eq_cnf}.}, label=formatCNF]

c Each comment line starts with "c"

c The CNF problem line is: "p" "cnf" $m $l
c   $m is the number of variables
c   $l is the number of clauses

c A CNF problem with 5 variables and 6 clauses:
p cnf 5 6

c Each clause line contains literals and ends with "0"

c A clause line with positive literals x1 and x3:
1 3 0

c A clause line with negative literals -x1 and -x3:
-1 -3 0

2 0

3 4 0

-4 0

5 0

\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Project-Join Tree}

Figure \ref{fig_jt_htb} illustrates a project-join tree $(T, n_{17}, \gamma, \pi)$ of the CNF formula $\phi$ in Equation \eqref{eq_cnf}.

\begin{figure}%[H]
    \centering
    \begin{tikzpicture} % use '~' for space; ' ' would crash
        \Tree [ .$n_{17}\overset\pi\mapsto\emptyset$
            [ .$n_{13}\overset\pi\mapsto\set{x_2}$ [ .$n_8\overset\pi\mapsto\emptyset$ [ .$n_3\overset{\gamma}{\mapsto}x_2$ ] ] ]
            [ .$n_{15}\overset\pi\mapsto\set{x_4}$
                [ .$n_{14}\overset\pi\mapsto\set{x_3}$
                    [ .$n_{12}\overset\pi\mapsto\set{x_1}$ [ .$n_7\overset\pi\mapsto\emptyset$
                        [ .$n_1\overset\gamma\mapsto{x_1 \vee x_3}$ ]
                        [ .$n_2\overset\gamma\mapsto{\neg x_1 \vee \neg x_3}$ ]
                    ] ]
                    [ .$n_9\overset\pi\mapsto\emptyset$ [ .$n_4\overset\gamma\mapsto{x_3 \vee x_4}$ ] ]
                ]
                [ .$n_{10}\overset\pi\mapsto\emptyset$ [ .$n_5\overset\gamma\mapsto{\neg x_4}$ ] ]
            ]
            [ .$n_{16}\overset\pi\mapsto\set{x_5}$ [ .$n_{11}\overset\pi\mapsto\emptyset$ [ .$n_6\overset\gamma\mapsto{x_5}$ ] ] ]
        ]
    \end{tikzpicture}
    \caption{
        In this project-join tree of the CNF formula in Equation \eqref{eq_cnf}, each leaf node ($n_1, \ldots, n_6$) corresponds to a unique clause, under the mapping $\gamma$.
        Each internal node ($n_7, \ldots, n_{17}$) corresponds to a distinct set of variables to project, under the mapping $\pi$.
    }
    \label{fig_jt_htb}
\end{figure}

See Listing \ref{formatJT} for the JT file format.

\begin{lstlisting}[float=*, firstline=2, caption={The join tree in Figure \ref{fig_jt_htb}.}, label=formatJT]

c Each comment line starts with "c"

c The join tree problem line is: "p" "jt" $m $l $n
c   $m is the number of CNF variables
c   $l is the number of CNF clauses
c   $n is the number of join tree nodes

c A join tree problem with 17 nodes:
c   6 leaf nodes
c   11 branch nodes (including 1 root node)
p jt 5 6 17

c Each leaf node corresponds to a unique CNF clause
c Leaf nodes are implicitly numbered 1 to $l

c Each branch node line is: $h $C "e" $P
c   $h is the index of the node ($l + 1 to $n)
c   $C lists indices of child nodes (1 to $h - 1)
c   $P lists variables that can be eliminated (1 to $m)

c Node 8 (branch node):
c   has 1 child, which is node 3 (leaf node)
c   eliminates no variable
8 3 e

c Node 13 (branch node):
c   has 1 child, which is node 8 (branch node)
c   eliminates variable 2
13 8 e 2

c Other branch node lines:
10 5 e
9 4 e
7 1 2 e
12 7 e 1
14 9 12 e 3
15 10 14 e 4
11 6 e
16 11 e 5

c Node 17 (root node):
17 13 15 16 e

\end{lstlisting}

